KAnoCLIP: Zero-Shot Anomaly Detection through Knowledge-Driven Prompt Learning and Enhanced Cross-Modal Integration

Zero-shot anomaly detection (ZSAD) identifies anomalies without needing training samples from the target dataset, essential for scenarios with privacy concerns or limited data. Vision-language models like CLIP show potential in ZSAD but have limitations: relying on manually crafted fixed textual descriptions or anomaly prompts is time-consuming and prone to semantic ambiguity, and CLIP struggles with pixel-level anomaly segmentation, focusing more on global semantics than local details. To address these limitations, We introduce KAnoCLIP, a novel ZSAD framework that leverages vision-language models. KAnoCLIP combines general knowledge from a Large Language Model (GPT-3.5) and fine-grained, image-specific knowledge from a Visual Question Answering system (Llama3) via Knowledge-Driven Prompt Learning (KnPL). KnPL uses a knowledge-driven (KD) loss function to create learnable anomaly prompts, removing the need for fixed text prompts and enhancing generalization. KAnoCLIP includes the CLIP visual encoder with V-V attention (CLIP-VV), Bi-Directional Cross-Attention for Multi-Level Cross-Modal Interaction (Bi-CMCI), and Conv-Adapter. These components preserve local visual semantics, improve local cross-modal fusion, and align global visual features with textual information, enhancing pixel-level anomaly detection. KAnoCLIP achieves state-of-the-art performance in ZSAD across 12 industrial and medical datasets, demonstrating superior generalization compared to existing methods.

==> sec/relatedwork.tex <==
\section{Related Works}

% \subsection{Large Vision-Language Models}
% \label{subsec:Large Vision-Language Models}
%   Large Vision-Language Models (LVLMs) have significantly advanced the integration of visual and textual data, exemplified by models like CLIP \cite{radford2021learning} and ALIGN \cite{jia2021align}, which use dual-encoder architectures for zero-shot image classification and retrieval. DALL-E and DALL-E 2 \cite{ramesh2022hierarchical} highlight the creative potential in text-to-image synthesis. Other notable advancements include Flamingo \cite{alayrac2022flamingo}, which combines Vision Transformers and large language models for multimodal tasks like image captioning and visual question answering, and BLIP \cite{li2022blip}, which leverages noisy web data for robust performance in image-text retrieval. PaLI \cite{chen2022pali} and GPT-4 \cite{achiam2023gpt} further illustrate the progress in handling diverse multimodal inputs and generating human-like text, showcasing the rapid development and varied applications of LVLMs in creative content generation and multimodal reasoning.
  
\subsection{Zero-Shot Anomaly Detection}
\label{subsec:Zero-Shot Anomaly Detection}
    Zero-shot anomaly detection (ZSAD) enables models to identify anomalies without training samples from the target dataset, addressing significant variations across different applications. Large vision-language models (LVLMs) have significantly advanced ZSAD. WinCLIP \cite{jeong2023winclip} used CLIP with domain-specific text prompts, April-GAN \cite{chen2023zero} mapped CLIP’s visual features to textual space for better integration, and MVFA-AD \cite{huang2024adapting} enhanced cross-modal fusion with a two-layer MLP. AnomalyCLIP \cite{zhou2023anomalyclip} introduced a class-agnostic learnable prompt but lacked fine-grained object descriptions. PromptAD \cite{li2024promptad} used a semantic cascading approach for few-shot detection with only normal samples, though it required significant manual effort and was sensitive to prompt changes.


\subsection{Prompt Learning}
\label{subsec:Prompt Learning}
   Context Optimization (CoOp) \cite{zhou2022learning} introduced learnable prompt texts for task-specific optimization but struggled with new class generalization. Conditional Context Optimization (CoCoOp) \cite{zhou2022conditional} improved by incorporating image-related information, though it faced overfitting with limited data. Visual Prompt Tuning (VPT) \cite{jia2022visual} and KgCoOp \cite{yao2023visual} introduced learnable visual prompts and minimized the distance between general and specific text embeddings, enhancing task generalization. DenseCLIP \cite{rao2022denseclip} extended these concepts to dense prediction tasks, improving accuracy by capturing finer-grained details essential for anomaly detection. AnomalyCLIP \cite{zhou2023anomalyclip} and PromptAD \cite{li2024promptad}demonstrated the effectiveness of prompt learning in zero-shot and few-shot anomaly detection, reducing the need for labeled data and making detection more practical and scalable.

   

==> tables/loss.tex <==
\begin{table}[]
% \Huge
\caption{The ablation results of joint optimization}
\label{tab:loss}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
 &  &  & \multicolumn{2}{c}{MVTec-AD} & \multicolumn{2}{c}{VisA} \\ \cmidrule(l){4-7} 
\multirow{-2}{*}{Global} & \multirow{-2}{*}{Local} & \multirow{-2}{*}{KD} & Image-AUC & Pixel-AUC & Image-AUC & Pixel-AUC \\ \midrule
\Checkmark & \XSolidBrush & \XSolidBrush & 51.0 & 77.4 & 60.1 & 80.3 \\
\XSolidBrush & \Checkmark & \XSolidBrush & 85.4 & 88.2 & 80.6 & 90.8 \\
\Checkmark & \Checkmark & \XSolidBrush & 90.2 & 92.9 & 81.3 & 92.2 \\
\Checkmark & \Checkmark & \Checkmark & {\color[HTML]{FE0000} \textbf{93.1}} & {\color[HTML]{FE0000} \textbf{94.3}} & {\color[HTML]{FE0000} \textbf{83.8}} & {\color[HTML]{FE0000} \textbf{97.7}} \\ \bottomrule
\end{tabular}
}
\end{table}
